Orion: A Unified Visual Agent for Multimodal Perception, Advanced Visual Reasoning and Execution

We introduce Orion, a visual agent that integrates vision-based reasoning with tool-augmented execution to achieve powerful, precise, multi-step visual intelligence across images, video, and documents. Unlike traditional vision-language models that generate descriptive outputs, Orion orchestrates a suite of specialized computer vision tools, including object detection, keypoint localization, panoptic segmentation, Optical Character Recognition (OCR), and geometric analysis, to execute complex multi-step visual workflows. The system achieves competitive performance across MMMU, MMBench, DocVQA, and MMLongBench while extending monolithic VLM capabilities to production-grade visual intelligence. Through its agentic, tool-augmented approach, Orion enables autonomous visual reasoning that bridges neural perception with symbolic execution, marking the transition from passive visual understanding to active, tool-driven visual intelligence. Try Orion for free at: https://chat.vlm.run Learn more at: https://www.vlm.run/orion

==> 4_use_cases_sections/use_cases.tex <==
\subsection{Real-World Applications}

\textbf{\texttt{Orion}} enables diverse applications across industries through its ability to orchestrate multiple specialized tools in automated workflows.

\subsubsection{Document Processing Automation}
Financial institutions process thousands of invoices, contracts, and forms daily. \textbf{\texttt{Orion}} can automatically extract key information (dates, amounts, parties), validate data completeness, flag anomalies, and generate structured reports—all in a single workflow that combines Optical Character Recognition (OCR), layout analysis, and data extraction tools.

\subsubsection{Medical Image Analysis}
Healthcare providers need to analyze medical images while ensuring patient privacy. \textbf{\texttt{Orion}} can detect anatomical structures, identify abnormalities, and generate structured reports while automatically redacting sensitive information (Protected Health Information, PHI) from images and documents.

\subsubsection{Accessibility Enhancement}
Creating accessible content requires describing images, transcribing videos, and extracting text from complex layouts. \textbf{\texttt{Orion}} automates these workflows, enabling content creators to generate alt-text, captions, and structured content descriptions at scale by combining image captioning, OCR, and video transcription tools.

\subsubsection{Quality Control in Manufacturing}
Manufacturing facilities can use \textbf{\texttt{Orion}} to automatically inspect products by detecting defects, measuring dimensions, reading serial numbers, and comparing results against specifications. The multi-step workflow combines object detection, OCR, and measurement tools in a single automated pipeline.

These examples illustrate how \textbf{\texttt{Orion}}'s ability to orchestrate multiple specialized tools enables workflows that would be impractical or impossible with traditional monolithic models.


==> evaluation_methodology_paragraph.tex <==
\paragraph{Human Evaluation Methodology and Bias Mitigation}
To ensure unbiased and reliable assessment of model outputs, we implement a comprehensive set of methodological safeguards. First, all model outputs are presented to evaluators with randomized labels (Model A, B, C, D) rather than revealing actual system identities, preventing bias from brand recognition or prior expectations. The assignment of labels to models is randomized independently for each evaluator, and the presentation order of outputs within each task is also randomized to prevent primacy and recency effects. Second, each task is evaluated by at least three independent evaluators who undergo calibration training on practice tasks to ensure consistent understanding of scoring criteria. We calculate inter-rater reliability and flag tasks with high disagreement (>20 percentage point variance) for additional review. Third, evaluators are selected from diverse backgrounds and work independently without discussion during evaluation sessions to prevent groupthink. Fourth, all evaluations are conducted under standardized conditions with consistent display settings and adequate time allocations. Fifth, we perform statistical outlier detection and sensitivity analyses to test robustness of results. Finally, we report inter-rater reliability metrics, confidence intervals, and methodological choices transparently. The evaluation employs a Composite Quality Score (0--100\%) calculated as a weighted average: task completion (0--100\%, weight 30\%), output accuracy (0--100\%, weight 35\%), visual quality (0--100\%, weight 20\%, when applicable), and task appropriateness (0--100\%, weight 15\%). Despite these safeguards, inherent limitations remain: some aspects of quality are subjective, and the selected task set may not represent all use cases. However, the combination of blinding, randomization, multiple evaluators, statistical controls, and transparency ensures that reported differences reflect genuine performance differences rather than methodological artifacts.


